"My nose is running.""Are you also coughing?": Building A Medical Diagnosis Agent with Interpretable Inquiry Logics

With the rise of telemedicine, the task of developing Dialogue Systems for Medical Diagnosis (DSMD) has received much attention in recent years. Different from early researches that needed to rely on extra human resources and expertise to help construct the system, recent researches focused on how to build DSMD in a purely data-driven manner. However, the previous data-driven DSMD methods largely overlooked the system interpretability, which is critical for a medical application, and they also suffered from the data sparsity issue at the same time. In this paper, we explore how to bring interpretability to data-driven DSMD. Specifically, we propose a more interpretable decision process to implement the dialogue manager of DSMD by reasonably mimicking real doctors' inquiry logics, and we devise a model with highly transparent components to conduct the inference. Moreover, we collect a new DSMD dataset, which has a much larger scale, more diverse patterns and is of higher quality than the existing ones. The experiments show that our method obtains 7.7%, 10.0%, 3.0% absolute improvement in diagnosis accuracy respectively on three datasets, demonstrating the effectiveness of its rational decision process and model design. Our codes and the GMD-12 dataset are available at https://github.com/lwgkzl/BR-Agent.

==> tab.tex <==
\begin{table*}[t]
% \setlength{\belowcaptionskip}{-0.4cm}
\centering
% \resizebox{\columnwidth}{!}{
\begin{tabular}{m{0.85cm}|m{2.5cm}|m{5cm}|m{5cm}}
\cmidrule[\heavyrulewidth]{1-4}
\textbf{Score} &\textbf{Description} & \textbf{Symptom Inquiry} & \textbf{Disease Diagnosis Report}
\\
%\textbf{Symptom Inquiry}& \textbf{Disease Diagnosis Cases}\\
\cmidrule{1-4}
5 & Very 

reasonable & \textbf{Suspected diseases:}

Esophagitis (0.93)

Dermatitis (0.08)

Rhinitis (0.08)

%\textbf{Inquiry Logic:}

%To ensure

\textbf{Queried symptom:}

Pharynx discomfort&

\textbf{Diagnosis disease:} Esophagitis

\textbf{Confidence level:} 0.96

%\textbf{Known symptoms:} Acid reflux (True), Pain behind the breastbone (True), Chest tightness (True)

\textbf{Supporting symptoms:} Acid reflux, Pain behind the breastbone, Chest tightness
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cmidrule{1-4}
4 & Reasonable & \textbf{Suspected diseases:}

Coronary heart disease (0.92)

Esophagitis (0.13)

Mastitis (0.08)

%\textbf{Inquiry Logic:}

%To distinguish

\textbf{Queried symptom:}

Acid reflux&

\textbf{Diagnosis disease:} Coronary Heart Disease

\textbf{Confidence level:} 0.65

%\textbf{Known symptoms:} Pain behind the breastbone (True), Stomach ache (False), Hematemesis (False)

\textbf{Supporting symptoms:} Pain behind the breastbone
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cmidrule{1-4}
3 & Seemingly 

reasonable & \textbf{Suspected diseases:}

Rhinitis (0.25)

Asthma (0.22)

Pneumonia (0.20)

%\textbf{Inquiry Logic:}

%To ensure

\textbf{Queried symptom:}

Cough&

\textbf{Diagnosis disease:} Asthma

\textbf{Confidence level:} 0.60

%\textbf{Known symptoms:} Consciousness disorder (True), Twitch (False), Cough (True), Expectoration (True)

\textbf{Supporting symptoms:} Expectoration, Cough
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cmidrule{1-4}
2 & Seemingly

unreasonable & \textbf{Suspected diseases:} 

Pneumonia (0.68)

Mastitis (0.22)

Asthma (0.15)

%\textbf{Inquiry Logic:}

%To distinguish

\textbf{Queried symptom:}

Sialorrhea & 

\textbf{Diagnosis disease:} Rhinitis

\textbf{Confidence level:} 0.27

%\textbf{Known symptoms:} Pharynx discomfort (True), Hemoptysis (True), Fever (False), Hard to swallow (False), Hoarse (False)

\textbf{Supporting symptoms:} Hoarse, hard to swallow, Hemoptysis, Pharynx discomfort
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cmidrule{1-4}
1 & Completely

unreasonable & \textbf{Suspected diseases:} 

external otitis (0.08) 

enteritis (0.08)

Traumatic brain injury (0.08)

%\textbf{Inquiry Logic:}

%To ensure

\textbf{Queried symptom:}

Cough & 

\textbf{Diagnosis disease:} Enteritis

\textbf{Confidence level:} 0.98

%\textbf{Known symptoms:} Stomach ache (True), Defecate (True), Night sweats (False), Fever (False)
\textbf{Supporting symptoms:} Stomach ache, Defecate
\\
\cmidrule[\heavyrulewidth]{1-4}
\end{tabular}
\caption{Samples of explanation reports for each rationality score. The ``Suspected diseases'' are the three most suspected diseases and their estimated probability. The cases in the last line are generated by the A2C-GCN baseline, while other cases are generated by our BR-Agent. }

\label{2}
\end{table*}
